Physics with first LHCb data

The LHCb experiment is designed for hadronic flavour physics and will look for New Physics manifestations in the decay of charm and bottom hadrons abundantly produced at the LHC. All parts of the LHCb physics programme can be embarked on with the expected statistics to be collected during the first 2010-2011 physics run at $\sqrt{s}$ = 7 TeV. We present first preliminary results on strangeness production, and demonstrate, using the few nb-1 of already collected data, the potential for initial measurements in heavy-flavour physics.

==> log <==
This is TeX, Version 3.14159 (Web2C 7.4.5)
(./schneider_olivier.tex
LaTeX2e <2001/06/01>
Babel <v3.7h> and hyphenation patterns for american, french, german, ngerman, n
ohyphenation, loaded.
(./desyproc.cls
Document Class: desyproc 2009/01/25 V1.0 DESY proceedings
(/usr/share/texmf/tex/latex/base/article.cls
Document Class: article 2001/04/21 v1.4e Standard LaTeX document class
(/usr/share/texmf/tex/latex/base/size10.clo))
(/usr/share/texmf/tex/latex/html/url.sty)
(/usr/share/texmf/tex/latex/graphics/graphicx.sty
(/usr/share/texmf/tex/latex/graphics/keyval.sty)
(/usr/share/texmf/tex/latex/graphics/graphics.sty
(/usr/share/texmf/tex/latex/graphics/trig.sty)
(/usr/share/texmf/tex/latex/config/graphics.cfg)
(/usr/share/texmf/tex/latex/graphics/dvips.def)))
(/usr/share/texmf/tex/latex/graphics/epsfig.sty)
(/usr/share/texmf/tex/latex/graphics/color.sty
(/usr/share/texmf/tex/latex/config/color.cfg)
(/usr/share/texmf/tex/latex/graphics/dvipsnam.def))
(/usr/share/texmf/tex/latex/misc/wrapfig.sty)
(/usr/share/texmf/tex/latex/misc/rotating.sty
(/usr/share/texmf/tex/latex/base/ifthen.sty))
(/usr/share/texmf/tex/latex/amsfonts/amssymb.sty
(/usr/share/texmf/tex/latex/amsfonts/amsfonts.sty))
(/usr/share/texmf/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/share/texmf/tex/latex/amsmath/amstext.sty
(/usr/share/texmf/tex/latex/amsmath/amsgen.sty))
(/usr/share/texmf/tex/latex/amsmath/amsbsy.sty)
(/usr/share/texmf/tex/latex/amsmath/amsopn.sty))
(/usr/share/texmf/tex/latex/tools/array.sty))
No file schneider_olivier.aux.
(/usr/share/texmf/tex/latex/amsfonts/umsa.fd)
(/usr/share/texmf/tex/latex/amsfonts/umsb.fd) [1]

LaTeX Warning: Citation `LHCb:2009ny' on page 2 undefined on input line 130.

<schneider_olivier.fig1a.eps> <schneider_olivier.fig1b.eps>

LaTeX Warning: Citation `Alves:2008zz' on page 2 undefined on input line 159.


LaTeX Warning: Reference `fig:LHCb' on page 2 undefined on input line 160.


LaTeX Warning: Reference `fig:LHCb' on page 2 undefined on input line 173.


LaTeX Warning: Citation `Golutvin_talk' on page 2 undefined on input line 202.


LaTeX Warning: Citation `Wiedner_talk' on page 2 undefined on input line 203.


LaTeX Warning: Citation `Maciuc_talk' on page 2 undefined on input line 204.


LaTeX Warning: Citation `Xing_talk' on page 2 undefined on input line 204.

[2] <schneider_olivier.fig2.eps>

LaTeX Warning: Reference `fig:W' on page 3 undefined on input line 235.


Underfull \hbox (badness 1484) in paragraph at lines 220--236
\OT1/cmr/m/n/10 and most abun-dantly pro-duced par-ti-cles.

LaTeX Warning: Citation `FerroLuzzi:2005em' on page 3 undefined on input line 2
42.


LaTeX Warning: Citation `Hopchev:2010tj' on page 3 undefined on input line 244.


<schneider_olivier.fig3a.eps>
Overfull \hbox (3.33333pt too wide) in paragraph at lines 252--254
[][] 
<schneider_olivier.fig3b.eps> <schneider_olivier.fig3c.eps>

LaTeX Warning: Citation `Skands_Perugia' on page 3 undefined on input line 275.



LaTeX Warning: Citation `Skands_Perugia' on page 3 undefined on input line 275.


[3]

LaTeX Warning: Reference `fig:Vzero' on page 4 undefined on input line 291.


LaTeX Warning: Reference `fig:Vzero' on page 4 undefined on input line 306.


LaTeX Warning: Citation `Kshort_paper' on page 4 undefined on input line 310.


Underfull \vbox (badness 1354) has occurred while \output is active [4]

LaTeX Warning: Citation `Bonivento_talk' on page 5 undefined on input line 314.



LaTeX Warning: Reference `fig:Vzero' on page 5 undefined on input line 317.

<schneider_olivier.fig4a.eps> <schneider_olivier.fig4b.eps>
<schneider_olivier.fig4c.eps> <schneider_olivier.fig4d.eps>
<schneider_olivier.fig4e.eps> <schneider_olivier.fig4f.eps>

LaTeX Warning: Reference `fig:charm' on page 5 undefined on input line 351.


LaTeX Warning: Citation `Marks_talk' on page 5 undefined on input line 354.

(/usr/share/texmf/tex/latex/base/omscmr.fd)

LaTeX Warning: Reference `fig:charm' on page 5 undefined on input line 362.


LaTeX Warning: Reference `fig:charm' on page 5 undefined on input line 369.


LaTeX Warning: Reference `fig:charm' on page 5 undefined on input line 386.

<schneider_olivier.fig5a.eps> <schneider_olivier.fig5b.eps> [5]
<schneider_olivier.fig6a.eps> <schneider_olivier.fig6b.eps>
<schneider_olivier.fig6c.eps> <schneider_olivier.fig6d.eps> [6]

LaTeX Warning: Reference `fig:Jpsi' on page 7 undefined on input line 438.


LaTeX Warning: Reference `fig:Jpsi' on page 7 undefined on input line 449.


LaTeX Warning: Reference `fig:Dzeromu' on page 7 undefined on input line 464.


LaTeX Warning: Citation `Dmu_paper' on page 7 undefined on input line 473.

[7] <schneider_olivier.fig7.eps>

LaTeX Warning: Reference `fig:Bexcl' on page 8 undefined on input line 496.


LaTeX Warning: Citation `LHCb:2009ny' on page 8 undefined on input line 504.

[8]

LaTeX Warning: Citation `LHCb:2009ny' on page 9 undefined on input line 511.

[9] (./schneider_olivier.aux)

LaTeX Warning: There were undefined references.


LaTeX Warning: Label(s) may have changed. Rerun to get cross-references right.

 )
(see the transcript file for additional information)
Output written on schneider_olivier.dvi (9 pages, 37836 bytes).
Transcript written on schneider_olivier.log.
This is TeX, Version 3.14159 (Web2C 7.4.5)
(./schneider_olivier.tex
LaTeX2e <2001/06/01>
Babel <v3.7h> and hyphenation patterns for american, french, german, ngerman, n
ohyphenation, loaded.
(./desyproc.cls
Document Class: desyproc 2009/01/25 V1.0 DESY proceedings
(/usr/share/texmf/tex/latex/base/article.cls
Document Class: article 2001/04/21 v1.4e Standard LaTeX document class
(/usr/share/texmf/tex/latex/base/size10.clo))
(/usr/share/texmf/tex/latex/html/url.sty)
(/usr/share/texmf/tex/latex/graphics/graphicx.sty
(/usr/share/texmf/tex/latex/graphics/keyval.sty)
(/usr/share/texmf/tex/latex/graphics/graphics.sty
(/usr/share/texmf/tex/latex/graphics/trig.sty)
(/usr/share/texmf/tex/latex/config/graphics.cfg)
(/usr/share/texmf/tex/latex/graphics/dvips.def)))
(/usr/share/texmf/tex/latex/graphics/epsfig.sty)
(/usr/share/texmf/tex/latex/graphics/color.sty
(/usr/share/texmf/tex/latex/config/color.cfg)
(/usr/share/texmf/tex/latex/graphics/dvipsnam.def))
(/usr/share/texmf/tex/latex/misc/wrapfig.sty)
(/usr/share/texmf/tex/latex/misc/rotating.sty
(/usr/share/texmf/tex/latex/base/ifthen.sty))
(/usr/share/texmf/tex/latex/amsfonts/amssymb.sty
(/usr/share/texmf/tex/latex/amsfonts/amsfonts.sty))
(/usr/share/texmf/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/share/texmf/tex/latex/amsmath/amstext.sty
(/usr/share/texmf/tex/latex/amsmath/amsgen.sty))
(/usr/share/texmf/tex/latex/amsmath/amsbsy.sty)
(/usr/share/texmf/tex/latex/amsmath/amsopn.sty))
(/usr/share/texmf/tex/latex/tools/array.sty)) (./schneider_olivier.aux)
(/usr/share/texmf/tex/latex/amsfonts/umsa.fd)
(/usr/share/texmf/tex/latex/amsfonts/umsb.fd) [1]
<schneider_olivier.fig1a.eps> <schneider_olivier.fig1b.eps> [2]
<schneider_olivier.fig2.eps>
Underfull \hbox (badness 1484) in paragraph at lines 220--236
\OT1/cmr/m/n/10 and most abun-dantly pro-duced par-ti-cles.
<schneider_olivier.fig3a.eps>
Overfull \hbox (3.33333pt too wide) in paragraph at lines 252--254
[][] 
<schneider_olivier.fig3b.eps> <schneider_olivier.fig3c.eps> [3]
Underfull \vbox (badness 1354) has occurred while \output is active [4]
<schneider_olivier.fig4a.eps> <schneider_olivier.fig4b.eps>
<schneider_olivier.fig4c.eps> <schneider_olivier.fig4d.eps>
<schneider_olivier.fig4e.eps> <schneider_olivier.fig4f.eps>
(/usr/share/texmf/tex/latex/base/omscmr.fd) <schneider_olivier.fig5a.eps>
<schneider_olivier.fig5b.eps> [5] <schneider_olivier.fig6a.eps>
<schneider_olivier.fig6b.eps> <schneider_olivier.fig6c.eps>
<schneider_olivier.fig6d.eps> [6] [7] <schneider_olivier.fig7.eps> [8] [9]
(./schneider_olivier.aux) )
(see the transcript file for additional information)
Output written on schneider_olivier.dvi (9 pages, 37692 bytes).
Transcript written on schneider_olivier.log.
This is dvips(k) 5.92b Copyright 2002 Radical Eye Software (www.radicaleye.com)
' TeX output 2010.10.09:1653' -> schneider_olivier.ps
<texc.pro><f7b6d320.enc><09fbbfac.enc><bbad153f.enc><aae443f0.enc>
<74afc74c.enc><0ef0afca.enc><10037936.enc><texps.pro><special.pro><color.pro>
. <cmbx8.pfb><cmti8.pfb><cmr8.pfb><cmbsy10.pfb><cmmib10.pfb><cmsy5.pfb>
<cmr5.pfb><cmsy7.pfb><cmmi7.pfb><cmr7.pfb><cmti10.pfb><cmsy10.pfb>
<cmmi10.pfb><cmbx12.pfb><cmr6.pfb><cmsy6.pfb><cmmi9.pfb><cmsy9.pfb><cmr9.pfb>
<cmtt10.pfb><cmbx10.pfb><cmr10.pfb><cmsl10.pfb>[1] [2
<schneider_olivier.fig1a.eps><schneider_olivier.fig1b.eps>] [3
<schneider_olivier.fig2.eps>] [4<schneider_olivier.fig3a.eps>
<schneider_olivier.fig3b.eps><schneider_olivier.fig3c.eps>] [5] [6
<schneider_olivier.fig4a.eps><schneider_olivier.fig4b.eps>
<schneider_olivier.fig4c.eps><schneider_olivier.fig4d.eps>
<schneider_olivier.fig4e.eps><schneider_olivier.fig4f.eps>] [7
<schneider_olivier.fig5a.eps><schneider_olivier.fig5b.eps>] [8
<schneider_olivier.fig6a.eps><schneider_olivier.fig6b.eps>
<schneider_olivier.fig6c.eps><schneider_olivier.fig6d.eps>] [9
<schneider_olivier.fig7.eps>] 

